When Modalities Conflict: How Unimodal Reasoning Uncertainty Governs Preference Dynamics in MLLMs

Multimodal large language models (MLLMs) must resolve conflicts when different modalities provide contradictory information, a process we term modality following. Prior work measured this behavior only with coarse dataset-level statistics, overlooking the influence of model's confidence in unimodal reasoning. In this paper, we introduce a new framework that decomposes modality following into two fundamental factors: relative reasoning uncertainty (the case-specific confidence gap between unimodal predictions) and inherent modality preference( a model's stable bias when uncertainties are balanced). To validate this framework, we construct a controllable dataset that systematically varies the reasoning difficulty of visual and textual inputs. Using entropy as a fine-grained uncertainty metric, we uncover a universal law: the probability of following a modality decreases monotonically as its relative uncertainty increases. At the relative difficulty level where the model tends to follow both modalities with comparable probability what we call the balance point, a practical indicator of the model's inherent preference. Unlike traditional macro-level ratios, this measure offers a more principled and less confounded way to characterize modality bias, disentangling it from unimodal capabilities and dataset artifacts. Further, by probing layer-wise predictions, we reveal the internal mechanism of oscillation: in ambiguous regions near the balance point, models vacillate between modalities across layers, explaining externally observed indecision. Together, these findings establish relative uncertainty and inherent preference as the two governing principles of modality following, offering both a quantitative framework and mechanistic insight into how MLLMs resolve conflicting information.

==> sections/3_behaviour_old.tex <==
\section{How MLLMs Make Decisions in Conflict Situations with Dynamic Unimodal difficulty }

\subsection{Dataset Construction}
\label{sec:methodology}

\noindent
To understand how unimodal reasoning difficulty influences modality preference when vision and text provide conflicting information, we construct controllable toy datasets in which vision and text can be independently manipulated. Each multimodal instance is indexed by a task type $\mathcal{T}$ and two categorical variables:
\[
x = \big(\, \mathcal{T},\, d_v,\, d_t \,\big),
\]
where $d_v$ denotes the visual difficulty level and $d_t$ the textual difficulty level. 
These variables represent stepwise increases in perceptual or reasoning demands, 
providing a stratified landscape in which difficulty can be systematically escalated.

% First, we introduce controllable toy datasets that allow unimodal difficulty to be varied in a structured way in Section~\ref{sec:conflict} (Section~\ref{sec:methodology}), then we show that conventional macro-level analyses of preference, although widely used, can be distorted by skewed difficulty distributions and thus produce misleading conclusions (Section~\ref{sec:illusion}). As a remedy, we propose a micro-level analysis on balanced difficulty landscapes, which reveals a robust S-shaped relation between preference and relative difficulty—an empirical characterization of the model’s decision function (Section~\ref{sec:scurve}). Finally, we extend this framework across models and tasks to validate its generality, and we introduce the notion of a \emph{task modulation effect}, which explains how task content dynamically shifts baseline preference (Section~\ref{sec:generalization}).

% \section{How the MLLM makes decisions in conflicting situations}
% \noindent
% This section presents a series of controlled experiments designed to uncover the mechanisms underlying modality preference in multimodal large language models (MLLMs). Our central hypothesis is that preference is not a static property of the model, but is dynamically shaped by the relative difficulty of unimodal reasoning. To investigate this, we construct a set of controllable benchmarks and introduce an \textit{entropy-based metric} that quantifies the model’s internal perception of difficulty (Section~\ref{sec:methodology}). 
% We then critically examine conventional macro-level analyses, showing that aggregated preference statistics are often distorted by skewed difficulty distributions and may lead to misleading conclusions (Section~\ref{sec:illusion}). As a remedy, we propose a micro-level analysis on a symmetrized, balanced difficulty landscape, which reveals a robust S-shaped relationship between modality preference and relative difficulty. This curve represents the model’s intrinsic decision function, disentangled from dataset biases (Section~\ref{sec:scurve}). Finally, we generalize this framework across multiple models and tasks, demonstrating its broad applicability and introducing the notion of a \textit{task modulation effect}, which explains how task content dynamically shifts baseline preference (Section~\ref{sec:generalization}).

% \subsection{Dataset Construction}
% \label{sec:methodology}

% \noindent
% To systematically probe modality preference, we implement a difficulty stratification framework. 
% Each multimodal instance is parameterized by two variables:
% \[
% x = \big(\, \mathcal{T},\, d_v,\, d_t \,\big),
% \]
% where $\mathcal{T}$ denotes the task type, $d_v$ the visual difficulty level, and $d_t$ the textual difficulty level.  
% Both $d_v$ and $d_t$ are categorical indices reflecting the number of steps 
% or perceptual load required to recover target information.

\paragraph{Color Recognition}
We take the color recognition task as an example. On the visual side, the baseline ($d_v=0$) contains only the target object, and difficulty($d_v=1 \to 10$) is
increased by shrinking the target, partially occluding it, or adding distractors. 
On the textual side, the baseline ($d_t=0$) is a direct conflicting statement (e.g.,
``The triangle is yellow''). Higher $d_t$ corresponds to requiring additional reasoning steps: 
explicit substitution ($d_t=1$, e.g., ``same color as the hexagon; the hexagon is yellow''), 
and implicit or multi-step substitution ($d_t=2$), which we instantiate using several strategies, 
including analogical color references (``same color as a morpho butterfly''), or shape-based reasoning 
(``the shape whose interior angles sum to $180^\circ$ is yellow,'' 
``the shape with three vertices,'' or ``the shape with three lines of symmetry''). Other tasks (shape counting, attribute recognition) follow the same paradigm, and a complete 
illustration of difficulty designs is provided in Appendix~\ref{app:difficulty}.

By pairing different levels of visual and textual difficulty, we generate a two-dimensional grid of multimodal instances. Each cell in this grid corresponds to a distinct difficulty configuration, thereby yielding a dataset that systematically spans a wide range of modality conflict scenarios. 



\subsection{Difficulty Measurement via Entropy}
\label{sec:entropy}

\noindent
To study how modality preference varies with \emph{continuous changes} in unimodal reasoning difficulty. we require an internal metric that directly reflects how difficult a given input is for the model itself. 
However, the dataset design in Section~\ref{sec:methodology} only provides a human-defined, stepwise notion of difficulty. Such design is not model-specific, nor sufficiently fine-grained to compare cases at the individual level. 

\paragraph{Entropy as the proxy of perceived difficulty.} 
Entropy has long been used in information theory and language model as a measure of uncertainty \citep{}. 
Intuitively, when the model is uncertain, the output distribution is diffuse (high entropy); 
when it is confident, the distribution is sharp (low entropy). This makes entropy a natural choice to quantify \emph{perceived difficulty}. 
\paragraph{Empirical validation.}  
We validate this metric on the color recognition dataset across multiple models and difficulty levels. 
Figure~\ref{fig:entropy_validation} shows that entropy is positively correlated with human-defined difficulty: 
accuracy decreases monotonically as difficulty increases, while the average entropy of correctly answered cases rises accordingly. 
We also observe that some incorrect cases exhibit low entropy (``confident mistakes''), whereas others show moderate entropy with fluctuating accuracy (``fragile knowledge''). 
Taken together, these results indicate that entropy provides a continuous, model-dependent, and case-level estimate of perceived difficulty, 
and we compute it primarily on correctly answered samples in all subsequent analyses.

% \paragraph{Unimodal evaluation.}  
% We estimate difficulty per modality by neutralizing the other:  
% \begin{itemize}
%     \item \textbf{Visual entropy:} $H^{(v)}$ is computed when the model answers with the image and a neutral text prompt.  
%     \item \textbf{Textual entropy:} $H^{(t)}$ is computed when the model answers with the text query and a blank image.  
% \end{itemize}
% For each case, we calculate the token-level entropy of the predictive distribution at the answer position, 
% providing a continuous estimate of confidence.  

% \paragraph{Empirical validation.}  
% We validate this metric on the color recognition dataset across different models and human-defined difficulty levels. 
% As shown in Figure~\ref{fig:entropy_validation}, entropy is strongly correlated with human-defined difficulty: 
% accuracy decreases monotonically with increasing difficulty, while the average entropy of correctly answered cases rises. 
% At the same time, two characteristic phenomena emerge:
% \begin{enumerate}
%     \item \textit{Confident mistakes:} low entropy despite incorrect answers, indicating overconfidence.  
%     \item \textit{Fragile knowledge:} moderate entropy coupled with unstable accuracy, revealing vulnerability to small perturbations.  
% \end{enumerate}
% These observations justify our methodological decision to focus on entropy computed from correctly answered samples, 
% so that it faithfully reflects perceived difficulty without contamination from spurious errors.  

% \begin{figure}[t]
%     \centering
%     % placeholder
%     \includegraphics[width=0.9\linewidth]{figures/entropy_validation.png}
%     \caption{Validation of entropy as a difficulty proxy on the color recognition dataset. 
%     Subplots show entropy distributions for correct vs.\ incorrect cases, and their relation to accuracy and human-defined difficulty levels.}
%     \label{fig:entropy_validation}
% \end{figure}

\begin{takeaways}
\textbf{Takeaways: }Entropy provides a model-dependent, case-level, and cross-modality comparable measure of perceived difficulty. 
It bridges the gap between human-defined difficulty design and the model’s internal uncertainty, 
and thus serves as the foundation for our subsequent analyses of modality preference.
\end{takeaways}


% \subsection{The Illusion of Aggregated Preference}
% \label{sec:illusion}

% \noindent
% A common practice in prior work is to measure modality preference by aggregating model choices 
% over the entire dataset, producing a single macro-level statistic such as the ``text-following rate.'' 
% While such numbers appear to provide a clear summary (e.g., ``LLaVA prefers text in 58\% of cases''), 
% they can in fact be misleading.

% \paragraph{Macro-level analysis.}
% We first follow this conventional approach and compute aggregated preference rates on our 
% original datasets without resampling. Table~\ref{tab:macro_pref} summarizes the results 
% for different models and tasks. These values suggest seemingly stable patterns of preference.

% \paragraph{Skewed difficulty distributions.}
% To understand what drives these macro statistics, we analyze the underlying difficulty landscape. 
% For each sample, we compute the entropy difference $\Delta H = H^{(t)} - H^{(v)}$ between text-only 
% and vision-only conditions, and plot the distribution for different models (Figure~\ref{fig:entropy_skew}). 
% We find that the distributions are highly skewed and vary substantially across models. 
% For instance, LLaVA tends to encounter more cases where $\Delta H < 0$ (vision easier), 
% whereas Qwen is exposed to cases with $\Delta H > 0$ (text easier).

% \paragraph{Takeaway.}
% These findings reveal that aggregated preference rates are confounded by the 
% skewness of difficulty distributions. What appears to be a ``true preference'' may 
% instead be an artifact of the dataset’s imbalance: the macro number is effectively 
% a weighted average of local decisions under biased conditions. This motivates the 
% need for a finer-grained, balanced analysis, which we develop in Section~\ref{sec:scurve}.



% \paragraph{Shape counting.}
% For task $\mathcal{T}=\text{Counting}$:
% \begin{itemize}
%     \item $d_v$: number of distractor objects in the image ($0$–$5$).
%     \item $d_t$: arithmetic reasoning complexity of the text statement.
%     \begin{align*}
%         d_t=0 &: X=2 \\
%         d_t=1 &: X=(2)+6 \\
%         d_t=2 &: X=((2)+6)-2 \\
%         d_t=3 &: X=(((2)+6)-2)+1
%     \end{align*}
% \end{itemize}

% \paragraph{Attribute recognition.}
% For task $\mathcal{T}=\text{Attribute}$ (based on CLEVR-style datasets):
% \begin{itemize}
%     \item $d_v$: image-level complexity (e.g., number of objects, object size).
%     \item $d_t$: textual indirection in attribute description (e.g., ``same material as a surgical glove'' instead of ``rubber'').
% \end{itemize}
